Rethinking Memory as Continuously Evolving Connectivity

Existing memory-augmented LLM agents often treat memory as a static repository with pre-defined representations and fixed retrieval pipelines, which is brittle in dynamic agentic environments where feedback, task variation, and heterogeneous signals continuously reshape what should be remembered and how it should be connected. To address this, we propose FluxMem, a connectivity-evolving memory framework that models memory as a heterogeneous graph and progressively refines its topology through three stages: initial connection formation, feedback-driven refinement, and long-term consolidation. During execution, FluxMem repairs missing links, prunes interference, aligns abstraction granularity, and distills recurrent successful trajectories into reusable procedural circuits, guided by one metric for memory generalizability and evolutionary maturity. Across three fundamentally distinct benchmarks including LoCoMo, Mind2Web, and GAIA, FluxMem achieves consistent state-of-the-art performance, demonstrating strong adaptation and generalization in complex agentic environments. The code will be open-sourced in https://github.com/zjunlp/LightMem.

==> section/memfactory.tex <==
\section{FluxMem}

\label{sec:method}

Unlike traditional memory systems that treat memory as a static repository of historical infomation, \textbf{FluxMem} treats memory as a dynamic representation that evolves through interaction and feedback. 
The system architecture is depicted in Figure~\ref{fig:architecture}. 
The core philosophy of \textbf{FluxMem} is to distill invariant knowledge, task-level experiences or robust skills from noisy, raw, and heterogeneous information across diverse scenarios. 

\subsection{Memory Schema and Evolutionary Metrics}
\label{preliminaries}
Rooted in the fundamentals of context engineering~\citep{mei2025surveycontextengineeringlarge} and actual agent-environment interaction patterns~\citep{yao2022react}, we define a four-level heterogeneous graph $G = (V, E)$ viewed through the lens of information flow. 
Ordered from base to apex, each level is characterized by specific node types: 

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figure/main_figure.png}
    \vspace{-0.4cm}
    \caption{The \textbf{FluxMem} architecture. \textbf{FluxMem} is architected as a four-layered heterogeneous graph. 
    Fundamentally distinguished from conventional knowledge graphs, it is engineered to accommodate a diverse array of intricate predefined scenarios.}
    \label{fig:architecture}
\end{figure*}

\begin{itemize}
    \item \textbf{Source Node ($V_{src}$):} The global corpus of raw information and environmental states, representing the agent's maximal exploration space. It encompasses all environmental inputs, such as complete dialogue histories, full HTML documents per step in web navigation, or entire code repositories. 
    \item \textbf{Evidence Node ($V_{evid}$):} Salient, task-specific snippets extracted from $V_{src}$ that filter out environmental noise to provide direct factual support for a particular query.
    \item \textbf{Episode Node ($V_{epi}$):} Detailed traces of individual task executions, recording the fine-grained interaction history, including the query, the intermediate reasoning steps, and the dynamic feedback, serving as the material for experience distillation.
    \item \textbf{Anchor Node ($V_{anc}$):} High-level, reusable abstractions (facts, experiences or skills) that are iteratively refined and gradually evolve from the joint synthesis of both the evidence and episode layers.
\end{itemize}

To govern the evolution of this graph, we introduce two core metrics: \textbf{Task-Evidence Distance (TED)} and \textbf{Anchor Evolution Maturity Score (AEMS)}.

\noindent \textbf{Task-Evidence Distance (TED).} To quantify the difficulty of memory generalization, we define TED to capture both semantic and functional discrepancies between task clusters. Recognizing that surface semantic similarity can be misleading, TED integrates query-level embeddings with the specific evidence nodes required for task resolution. For two clusters $C_i$ and $C_j$, the distance is formulated as:

\begin{equation}
TED(C_i, C_j) = \underbrace{(1 - \frac{\mathbf{\bar{q}}_i \cdot \mathbf{\bar{q}}_j}{\|\mathbf{\bar{q}}_i\| \|\mathbf{\bar{q}}_j\|})}_{\text{Query Distance}} + \underbrace{(1 - \frac{|E_{set,i} \cap E_{set,j}|}{|E_{set,i} \cup E_{set,j}|})}_{\text{Evidence Distance}}
\end{equation}

where $\mathbf{\bar{q}}$ denotes the arithmetic centroid of query embeddings within a task cluster, and $E = \{e \in V_{evid} \mid e \text{ is evidence node utilized by queries in } C\}$ represents the set of evidence nodes invoked during task execution. This dual-perspective metric ensures a robust measure of task relatedness, guiding the generalization and evolution mechanisms detailed in~\ref{phase1} and~\ref{phase3}, respectively.

\noindent \textbf{Anchor Evolution Maturity Score (AEMS).} We evaluate the quality of the evolved anchor nodes $V_{anc}^{(k)}$ at the $k$-th iteration by balancing their functional utility, information compactness, and semantic stability. The maturity score $\mathcal{M}_k$ is formulated as:
\begin{equation}
\mathcal{M}_k = \frac{\eta(V_{anc}^{(k)})}{\log \ell(V_{anc}^{(k)})} \times (1 - \delta(V_{anc}^{(k)}, V_{anc}^{(k-1)}))
\end{equation}
where $\eta(V_{anc}^{(k)})$ denotes the performance, measured by the joint success rate of the current anchor set across both the original and newly incorporated tasks, $\ell(V_{anc}^{(k)})$ represents the total token consumption to account for the efficiency, and $\delta(V_{anc}^{(k)}, V_{anc}^{(k-1)})$ quantifies the semantic drift, measuring the displacement in the embedding space between successive iterations. Evolution terminates when $\mathcal{M}_k$ plateaus.

\subsection{Phase I: Task Space Exploration and Anchor Inheritance}
\label{phase1}
Upon receiving a new query $q$, \textbf{FluxMem} does not treat the query as isolated point. Instead, it expands the query into a task-oriented cluster to explore the local information entropy and latent task space.

\noindent \textbf{Task Cluster Expansion.} Given an initial query $q_0$, we generate a task cluster $C_q = \{q_0, q_1, ..., q_n\}$ through three orthogonal perturbation strategies: 
(1) \textit{Surface Expansion:} Generates semantic paraphrases to mitigate sensitivity to lexical variations, 
(2) \textit{Structural Expansion:} Decomposes complex queries into sub-questions to capture compositional dependencies, 
and (3) \textit{Variable Expansion:} Perturbs numerical or entity-specific parameters to identify decision boundaries.
Let $\mathcal{E}_{exp}$ be the set of evidences retrieved for $\mathcal{C}_{q}$. 
This expansion transforms $q_0$ from an isolated point into a localized task neighborhood, enabling the memory system to achieve \textbf{preliminary task generalization}. 
Crucially, while a single query often provides limited retrieval cues, potentially missing certain golden evidences. 
By diversifying query variables and decomposing complex intents into sub-problems, we provide \textbf{more comprehensive yet targeted retrieval cues}, where sub-questions sharpen the retrieval focus on specific logical components, thereby increasing the diversity of retrieved results and the probability of covering the complete set of golden evidences required for the task. 

\noindent \textbf{Anchor Inheritance.} Instead of starting from scratch, $C_{q}$ calculates its $TED$ against existing clusters in the graph:
We first identify the set of $K$ nearest task clusters $\mathcal{K} \subseteq \mathcal{C}_{q}$ with respect to $C_{q}$ using the $TED$ metric. The inherited anchors are then retrieved as:
\begin{equation}
\mathcal{A}_{inherited} = \{ a \in V_{anc} \mid \text{is\_linked}(a, C), C \in \mathcal{K} \}
\end{equation}
By leveraging anchors associated with proximal task clusters, the agent incorporates supplementary background context and historical experiences from similar tasks into the current task to enhance its ability to navigate complex queries through cross-task insights. 

\noindent \textbf{Anchor-Guided Reasoning.} Agent executes current task using the retrieved evidences $\mathcal{E}_{exp}$ and inherited anchors $\mathcal{A}_{inherited}$. 
The response is generated as $R = f_{LLM}(C_q, \mathcal{E}_{exp}, \mathcal{A}_{inherited})$.


\subsection{Phase II: Error Correction and Reflection Leveraging Failure Memory}
\label{phase2}

Upon receiving a failure signal from the environment, \textbf{FluxMem} triggers an \textit{Failure-Driven Attribution and Refinement} mechanism to perform a root-cause analysis of the execution context.

If the failure is attributed to \textbf{information deficiency} by agent itself, the agent expands its search space by either re-initiating a deep retrieval from the source nodes $V_{src}$ or increasing the inheritance breadth $K$ in the \textit{Anchor Inheritance} phase to incorporate more guiding anchors. Conversely, if the error stems from \textbf{semantic redundancy} or misleading information (hallucination), the agent adopts a conservative strategy by severing all connections to inherited anchors and relying exclusively on evidence nodes $V_{evid}$ to eliminate distractions: 
\begin{equation}
\mathcal{E}' = 
\begin{cases} 
f_{search}(V_{src}, \text{expand}(K)), & \text{if } \text{Deficiency} \\
\{e \in \mathcal{E} \mid \text{is\_relevant}(e, q)\}, & \text{if } \text{Redundancy}
\end{cases}
\end{equation}

Simultaneously, the agent encapsulates the failed interaction trajectory $\tau_{fail}$ into the anchor nodes, which serves as a cautionary constraint for future tasks of the same type:
\begin{equation}
V_{anc} \leftarrow V_{anc} \cup \{ \text{distill}(\tau_{fail}) \}
\end{equation} 
where the distillation process extracts specific ``don't do'' instructions from the failure. By integrating these reorganized evidences and negative experiences, the agent re-executes the reflection process until success or a maximum step limit ($T_{max}$) is reached before moving to the evolution phase. 

\subsection{Phase III: Offline Continuous Evolution}
\label{phase3}
To prevent the memory from degenerating into a cluttered and unmanageable collection of disjointed episodes, \textbf{FluxMem} undergoes a phase of periodic offline evolution.

\noindent \textbf{Clustering and Induction.} When the number of new episode nodes $|V_{epi}|$ (task cluster) exceeds a threshold $\tau$, we perform global clustering based on $TED$. For each cluster, we invoke an induction operator $f_{LLM}$ to extract invariant patterns (anchors):
\begin{equation}
V_{anc}^{(k)} = \mathcal{f}_{\text{LLM}}(V_{epi}, V_{evid} \subseteq G)
\end{equation}
This operator distills common reasoning steps, frequent error-correction patterns, and optimal context organizations into new or updated anchor nodes.

\noindent \textbf{Iterative Evolution.} The evolution of memory within \textbf{FluxMem} is conceptualized as a multi-round refinement rather than a single-pass extraction. 
The system iteratively updates the anchor set $V_{anc}^{(k)}$ and re-evaluates the maturity score $\mathcal{M}_k$ to monitor the evolutionary trajectory. 
A new induction cycle is triggered as long as the marginal improvement in maturity $\Delta \mathcal{M}$ exceeds a sensitivity threshold $\epsilon$ and the semantic drift $\delta$ remains above a stability tolerance $\tau$, indicating that the knowledge structure has not yet reached its optimal equilibrium. 
Conversely, when these metrics stabilize, the anchors are deemed ``crystallized'', they transition into a state of epistemic invariance, representing the most stable, token-efficient, and robust task-solving kernels. 

Through this recursive evolutionary cycle, \textbf{FluxMem} successfully distills stochastic, high-variance interaction traces into a structured, hierarchical knowledge base, empowering the agent with superior adaptive capabilities in highly dynamic and unstable environments.

==> section/method.tex <==
\section{Memory Graph Formalization}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figure/mmexport1776062418337.jpg}
    \vspace{-0.4cm}
    \caption{The \textbf{MemFactory} architecture. \textbf{MemFactory} is architected as a four-layered heterogeneous graph. 
    Fundamentally distinguished from conventional knowledge graphs, it is engineered to accommodate a diverse array of intricate predefined scenarios.}
    \label{fig:architecture}
\end{figure*}

\subsection{Graph Architecture and Node Taxonomy}
Formally, $M$ is structured as a four-tier heterogeneous graph $G=(V,\mathcal{E})$. 
Distinct from static knowledge graphs that prioritize factual completeness, this structure is designed to support dynamic context induction, where nodes encapsulate heterogeneous information types and functional roles, while edges encode the evolving connectivity required for task-adaptive reasoning.
As shown in Figure~\ref{fig:architecture}, the node set $V$ is organized into a hierarchy that mirrors the agent's information processing pipeline from raw perception to abstract reasoning. 
Crucially, each node materializes as a concrete context fragment such as raw text spans, structured execution logs, or templated skill instructions that is directly serializable and injectable into the model's prompt, thereby grounding the memory graph in practical implementation rather than abstract conceptualization. 
(i) \textbf{Source Nodes ($V_{src}$)} constitute the foundational layer, encompassing the agent's maximal exploration space of raw environmental states (e.g., full HTML documents, complete code repositories, or unfiltered dialogue histories). 
(ii) \textbf{Evidence Nodes ($V_{evid}$)} form the primary retrieval tier, consisting of salient, task-specific snippets filtered from $V_{src}$ that directly map to the factual evidence component $E_t(q)$. 
(iii) \textbf{Episode Nodes ($V_{epi}$)} capture fine-grained execution trajectories, recording queries, intermediate reasoning steps, and dynamic feedback to instantiate the historical episode component $H_t(q)$. 
(iv) \textbf{Anchor Nodes ($V_{anc}$)} reside at the apex, representing high-level, reusable abstractions distilled from recurrent evidence and successful episodes, which directly correspond to the procedural skill component $P_t(q)$. 
While $V_{src}$ grounds the memory in environmental reality, the upper triad of $V_{evid}$, $V_{epi}$, and $V_{anc}$ constitutes the active substrate dynamically assembled into the context state $S_t(q)$. 

\subsection{Context State as an Induced Subgraph}
For task $q$ at step $t$, the context state $S_t(q)$ is defined as a \emph{dynamically induced local subgraph} $G_t(q) = (V_t, \mathcal{E}_t) \subset G$, where $V_t = V_t^{evid} \cup V_t^{epi} \cup V_t^{anc}$. 
The context construction process $\mathcal{C}(\cdot)$ operates by querying $G$ with $O_t(q)$, traversing relevant edges to activate $V_t$, and linearizing the relational topology into the prompt. 
Thus, optimizing $S_t(q)$ is equivalent to performing targeted topological edits on $G_t(q)$, where node selection, edge activation, and subgraph density directly determine reasoning efficacy.

\subsection{Atomic Context Operations}

\label{atomic_operation}
To formalize the adaptation pipeline, we define primitive graph operators that directly instantiate the optimization objectives outlined in Problem Formulation. These operators are structured to sequentially address the intra-task refinement challenges and the inter-task evolution requirement:
\begin{enumerate}
    \item \textbf{Component Gating ($\text{Bypass}$):} Addresses the necessity of memory modules. $\text{Bypass}(G_t)$ temporarily suppresses $\{V_t^{evid}, V_t^{epi}, V_t^{anc}\}$, isolating $O_t(q)$ to eliminate unnecessary cognitive overhead when steps are purely environment-grounded.
    \item \textbf{Retrieval Fidelity ($\text{Prune}$ or $\text{Expand}$):} Addresses signal-to-noise imbalances within active components. $\text{Prune}(G_t)$ identifies and removes low-relevance or contradictory nodes from $V_t$ to purge semantic interference, while $\text{Expand}(G_t, q)$ queries the broader graph for missing critical evidence or skills to recover structural deficiency.
    \item \textbf{Granularity Alignment ($\text{Align}$):} Addresses abstraction mismatches by adjusting the granularity of $\{E_t, H_t, P_t\}$ to match the precision required by $O_t(q)$. $\text{Align}(G_t, \lambda)$ substitutes nodes with granularly matched alternatives from adjacent layers (parameterized by abstraction level $\lambda$), ensuring optimal context alignment with reasoning demands.
    \item \textbf{Structural Evolution ($\text{Induce}$):} Addresses long-term memory sustainability and recurrent error prevention. $\text{Induce}(\tau, G)$ extracts invariant causal patterns from the trajectory $\tau$, updating anchor nodes $V_{anc}$ to internalize successful context-action mappings. This operation explicitly minimizes the divergence between future initial contexts $S_1(q')$ and optimal states, thereby reducing future refinement costs $\mathcal{C}_{\text{ref}}$.
\end{enumerate}
Collectively, the first three categories instantiate the intra-task refinement operator $\mathcal{T}(\cdot)$, while the fourth instantiates the inter-task evolution operator $\mathcal{U}(\cdot)$, transforming the abstract optimization objectives into concrete, executable graph manipulations.


\section{Two-Level Adaptive Context Evolution}

Building upon the graph substrate defined above, MemFactory operationalizes the two-level adaptation framework as a closed-loop pipeline. For each task $q$, the system first induces a comprehensive initial context state, then iteratively refines it via environmental feedback, and finally consolidates successful patterns into the persistent graph. 

\subsection{Initial Context Induction}
For each task $q$, the system constructs an initial context state $S_1(q)$ via a deterministic, three-stage retrieval and graph-induction process directly from the task $q$: 

\paragraph{Stage 1: Evidence Extracting.} The query $q$ probes the source layer $V_{src}$ to instantiate factual evidence nodes. We compute a hybrid relevance score for each $v \in V_{src}$ by combining dense, sparse, and LLM-based signals:
\[
\text{Score}(v, q) = \alpha \cdot \frac{\mathbf{v} \cdot \mathbf{q}}{\|\mathbf{v}\| \|\mathbf{q}\|} + \beta \cdot \text{BM25}(v, q) + \gamma \cdot \text{LLM}_{\text{rel}}(v, q),
\]
where $\alpha+\beta+\gamma=1$, and $\text{LLM}_{\text{rel}}(v, q) \in \{0, 1\}$ is a binary relevance judgment obtained by directly prompting the LLM to verify whether $v$ contains necessary evidence for $q$. The top-$k$ source snippets are extracted and instantiated as evidence nodes $E_1 \subset V_{evid}$, with retrieval edges added to the graph:
\[
\mathcal{E} \leftarrow \mathcal{E} \cup \{(e, v) \mid e \in E_1, v \in \text{TopK}_{v \in V_{src}}\{\text{Score}(v, q)\}\}.
\]

\paragraph{Stage 2: Episode Initialization \& Historical Retrieval.} 
For the current task $q$, we instantiate a dedicated episode node $v_q \in V_{epi}$ to record its execution trace, and establish causal edges to the retrieved evidence:
\[
V \leftarrow V \cup \{v_q\}, \quad \mathcal{E} \leftarrow \mathcal{E} \cup \{(v_q, e) \mid e \in E_1\}.
\]
Distinct from prior approaches that rely solely on static evidence, our method additionally retrieves historical task episodes similar to $q$ from $V_{epi}$. These traces $H_1 \subset V_{epi}$ are incorporated into the context to provide concrete execution guidance based on analogous past tasks. Formally, the historical set is retrieved via embedding similarity:
\[
H_1 = \text{TopK}_{u \in V_{epi} \setminus \{v_q\}} \big\{ \cos(\mathbf{u}, \mathbf{q}) \big\}.
\]

\paragraph{Stage 3: Anchor Inheritance.} 
The retrieved historical episodes $H_1$ serve as retrieval keys for high-level procedural knowledge. Each $u \in H_1$ maintains directed edges in $\mathcal{E}$ to the anchor nodes $a \in V_{anc}$ that encapsulate the core skills or reasoning templates used during its execution. We aggregate these parent anchors to form the initial skill guidance set $P_1$. Formally, this inheritance is defined as:
\[
P_1 = \big\{ a \in V_{anc} \mid \exists u \in H_1, (a, u) \in \mathcal{E} \big\}.
\]

\paragraph{Context Assembly.} The induced components are linearized into the initial context state:
\[
S_1(q) = \mathcal{C}\big(O_1(q), E_1, H_1, P_1\big).
\]
While this pipeline establishes a structured baseline, the initial subgraph $G_1(q)$ inherently suffers from retrieval sparsity or granularity misalignment, necessitating the feedback-driven refinement loop detailed below.

\subsection{Feedback-Driven Context Refinement}
This phase instantiates the intra-task refinement operator $\mathcal{T}(\cdot)$ via a Reflexion-style closed loop: \emph{execute} $\to$ \emph{feedback/reflect} $\to$ \emph{attribute} $\to$ \emph{act}. Given the current episode node $v_q$ and its induced context subgraph, the process unfolds as follows:

\paragraph{Execution and Feedback Generation.}
The agent generates an action $a_t$ conditioned on the current context $S_t(q)$. It first attempts to acquire external environmental feedback $f_t^{\text{ext}}$. If $f_t^{\text{ext}}$ is unavailable or ambiguous, the agent triggers a self-verification prompt to evaluate the correctness of $a_t$, yielding a unified feedback signal $f_t$.

\paragraph{Hierarchical Attribution and Topology Mapping.}
Upon receiving $f_t$, the agent triggers a self-reflection process to diagnose the root cause of execution failure. This reflection sequentially evaluates three contextual dimensions, mapping the self-attributed issue to a specific graph topology edit:
\begin{itemize}
    \item \textbf{Necessity Check $\to$ Bypass:} The model first reflects on whether memory augmentation was actually required for $a_t$. If the reflection concludes that the step is purely environment-grounded and memory components only introduce latency or conflict, the system isolates $v_q$ from $\{E_t, H_t, P_t\}$ by temporarily masking their incident edges in $\mathcal{E}$.
    \item \textbf{Fidelity Check (Deficiency) $\to$ Expand:} If memory is deemed necessary but the execution failed, the model reflects on whether critical information was missing. Upon attributing the failure to a factual or procedural gap, the system relaxes the retrieval threshold (or increases $k$), identifies new candidate nodes $e_{\text{new}} \in V_{\text{evid}} \cup V_{\text{anc}}$, and establishes new causal edges:
    \[
    \mathcal{E} \leftarrow \mathcal{E} \cup \{(v_q, e_{\text{new}})\}.
    \]
    \item \textbf{Fidelity Check (Interference) $\to$ Prune:} Alternatively, if the reflection attributes the failure to hallucinated or contradictory guidance (context rot), the system identifies low-confidence nodes $e_{\text{noise}}$ within the current subgraph and severs their connections to $v_q$:
    \[
    \mathcal{E} \leftarrow \mathcal{E} \setminus \{(v_q, e_{\text{noise}})\},
    \]
    purging distractor signals from the prompt.
    \item \textbf{Granularity Check $\to$ Align:} If fidelity is sufficient but the reflection indicates reasoning rigidity or prompt congestion, the failure is attributed to an abstraction mismatch. The system substitutes nodes across layers (e.g., replacing an abstract anchor $a$ with a concrete historical episode $e'$), updating the edge set via edge swapping:
    \[
    \mathcal{E} \leftarrow \big(\mathcal{E} \setminus \{(v_q, a)\}\big) \cup \{(v_q, e')\}.
    \]
\end{itemize}

\paragraph{Context Reconstruction and Re-execution.}
After the topology is modified, the refined context state is reconstructed by linearizing the updated subgraph $G'_t(q) = (V_t, \mathcal{E}'_t)$:
\[
S'_t(q) = \mathcal{C}\big(O_t(q), G'_t(q)\big).
\]
The agent re-executes the step using $S'_t(q)$. This loop iterates until $f_t$ signals success or a maximum trial limit $T_{\max}$ is reached, guaranteeing that every context transition is explicitly driven by model-reflected attribution through concrete graph edits.


\subsection{Inter-Task Memory Evolution}
While $\mathcal{T}(\cdot)$ optimizes transient performance, long-term capability requires evolving the persistent graph $G$ via the operator $\mathcal{U}(\cdot)$. This phase prevents recurrent cognitive errors by internalizing successful context patterns across tasks.

\paragraph{Trajectory Write-Back.}
Upon task completion, the agent records the refined trajectory $\tau = \{(S'_t, a_t, f_t)\}_{t=1}^T$ as a new episode node $v_{epi}^{new} \in V_{epi}$. Directed edges are established linking $v_{epi}^{new}$ to all utilized evidence $V_t^{evid}$ and anchors $V_t^{anc}$, preserving the causal provenance of the successful reasoning path.

\paragraph{Periodic Consolidation via Induction.}
When the accumulation of new episodes exceeds a threshold $\tau_{\text{cons}}$, the system triggers offline consolidation. Successful trajectories are clustered by task similarity, and the induction operator extracts invariant reasoning patterns to update anchor nodes:
\[
V_{anc}^{new} = \text{Induce}\big(\{v \in V_{epi} \mid v \in \mathcal{C}_{\text{cluster}}\}, G\big).
\]
This operation elevates recurrent, high-utility subgraph configurations into stable procedural knowledge, effectively caching the optimal outputs of $\mathcal{T}(\cdot)$ for future retrieval.

\paragraph{Evolution Convergence.}
Consolidation proceeds iteratively until the graph reaches epistemic stability, monitored by the \emph{Anchor Evolution Maturity Score (AEMS)}:
\[
\text{AEMS}^{(k)} = \frac{\eta(V_{anc}^{(k)})}{\log \ell(V_{anc}^{(k)})} \times \big(1 - \delta(V_{anc}^{(k)}, V_{anc}^{(k-1)})\big),
\]
where $\eta$ measures cross-task success utility, $\ell$ denotes token footprint, and $\delta$ quantifies semantic drift. When $\Delta \text{AEMS} < \epsilon$, evolution halts and $G$ is deemed crystallized. At this equilibrium, the memory evolution operator satisfies $M_{k+1} = \mathcal{U}(M_k, \tau_k, f_{\text{final}})$, and the system achieves long-term sample efficiency: initial context states $S_1(q')$ for future tasks are inherently proximal to optimal configurations, drastically reducing the reliance on costly intra-task refinement.

